CPM: Class-conditional Prompting Machine for Audio-visual Segmentation

Audio-visual segmentation (AVS) is an emerging task that aims to accurately segment sounding objects based on audio-visual cues. The success of AVS learning systems depends on the effectiveness of cross-modal interaction. Such a requirement can be naturally fulfilled by leveraging transformer-based segmentation architecture due to its inherent ability to capture long-range dependencies and flexibility in handling different modalities. However, the inherent training issues of transformer-based methods, such as the low efficacy of cross-attention and unstable bipartite matching, can be amplified in AVS, particularly when the learned audio query does not provide a clear semantic clue. In this paper, we address these two issues with the new Class-conditional Prompting Machine (CPM). CPM improves the bipartite matching with a learning strategy combining class-agnostic queries with class-conditional queries. The efficacy of cross-modal attention is upgraded with new learning objectives for the audio, visual and joint modalities. We conduct experiments on AVS benchmarks, demonstrating that our method achieves state-of-the-art (SOTA) segmentation accuracy.

==> tables/ablation_gmm.tex <==
% \begin{minipage}[b]{0.5\textwidth}
% \begin{table}[t]
\begin{wraptable}{r}{0.54\linewidth}
% \centering
\vspace{-15pt}
\caption{Ablation of distribution representation modelling on AVSBench-Semantic~\cite{liu2023audio}.}
% \def\arraystretch{1.1}
% \resizebox{1.\linewidth}{!}{%
% \begin{tabular}{
\begin{tabular}{l||m{40pt}|m{40pt}}
% !{\vrule width 1.2pt}c!{\vrule width 1.2pt}P{50pt}|P{50pt}|P{50pt}|P{50pt}
% !{\vrule width 1.2pt}
% !{\vrule width 1.2pt}P{100pt}|P{70pt}!{\vrule width 1.2pt}
% } 
\specialrule{1.2pt}{0pt}{0pt}
% \multirow{2}{*}{Method} & \multicolumn{2}{c|}{AVSBench-Semantics} & \multicolumn{2}{c!{\vrule width 1.2pt}}{VPO (MSMI)} \\
% \multirow{1}{*}{Method} & \multicolumn{1}{c|}{AVSBench-Semantics}  \\
% \multicolumn{5}{!{\vrule width 1.2pt}c!{\vrule width 1.2pt}}{Method} & \multicolumn{2}{c!{\vrule width 1.2pt}}{Metrics}  \\ \hline
Method & mIoU & $F_{\beta}$ \\ \hline
Point Representation & 55.96 & 68.58 \\
Dist Representation & 57.25 & 70.54 \\
\specialrule{1.2pt}{0pt}{0pt}
% \specialrule{1.2pt}{0pt}{0pt}
Num Components & mIoU & $F_{\beta}$ \\ \hline
1 & 55.83 & 68.68 \\
3 & 57.25 & 70.54 \\
5 & 56.31 & 69.04 \\
7 & 56.05 & 68.59 \\
% 
\specialrule{1.2pt}{0pt}{0pt}
\end{tabular}
\label{tab:ablation_gmm}
% }
\vspace{-25pt}
% \end{table}    
\end{wraptable} 





